Domain Generalization in Computational Pathology: Survey and Guidelines

Deep learning models have exhibited exceptional effectiveness in Computational Pathology (CPath) by tackling intricate tasks across an array of histology image analysis applications. Nevertheless, the presence of out-of-distribution data (stemming from a multitude of sources such as disparate imaging devices and diverse tissue preparation methods) can cause \emph{domain shift} (DS). DS decreases the generalization of trained models to unseen datasets with slightly different data distributions, prompting the need for innovative \emph{domain generalization} (DG) solutions. Recognizing the potential of DG methods to significantly influence diagnostic and prognostic models in cancer studies and clinical practice, we present this survey along with guidelines on achieving DG in CPath. We rigorously define various DS types, systematically review and categorize existing DG approaches and resources in CPath, and provide insights into their advantages, limitations, and applicability. We also conduct thorough benchmarking experiments with 28 cutting-edge DG algorithms to address a complex DG problem. Our findings suggest that careful experiment design and CPath-specific Stain Augmentation technique can be very effective. However, there is no one-size-fits-all solution for DG in CPath. Therefore, we establish clear guidelines for detecting and managing DS depending on different scenarios. While most of the concepts, guidelines, and recommendations are given for applications in CPath, we believe that they are applicable to most medical image analysis tasks as well.

==> old_Stuff.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% OLD dataset table
\onecolumn
%\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.2} 
\begin{center}
\begin{longtable}
{p{4cm}p{3cm}p{3cm}p{5cm}}
\caption{Domain Generalization Datasets}
\label{table:datasets} \\
 \hline
 \textbf{Dataset} & \textbf{Task/Application} & \textbf{Domain Shift } & \textbf{No. of Domains}\\
 \hline 
 \endfirsthead
 \multicolumn{4}{c}%
{{\tablename\ \thetable{} -- continued from previous page}} \\
\hline
\textbf{Dataset} & \textbf{Task/Application} & \textbf{Domain Shift } & \textbf{No. of Domains} \\
\hline
\endhead

\hline \multicolumn{4}{r}{{Continued on next page}} \\ \hline
\endfoot

\hline
\endlastfoot
\multicolumn{4}{|c|}{\textbf{Detection}}\\
\hline
Mitosis Domain Generalization Challenge 2021 (MIDOG21) \cite{64_aubreville2023cpath} & Mitosis Classification & Type 1 & Six different domains owing to the use of six different scanners across the entire dataset. \\ 
\hline
 Mitosis Domain Generalization Challenge 2022 (MIDOG22) \cite{65_aubreville2022cpath} \cite{midog22dataset} & Mitosis Classification & Type 1, Type 2, Type 3 &  Six different domains due to the presence of cases from different tumor types (from species and scanned by different scanners). \\ 
 \hline
A comprehensive multi-domain dataset for mitotic figure detection (MIDOG++) & Mitosis Classification & Type 1, Type 2, Type 3 & Seven different domains with respect to tumor types \\ 
 \hline
 MITOS-ATYPIA-14 \cite{126_roux2014_cpath} & Mitosis Classification & Type 1 &  Two domains as the dataset consisted of cases scanned using two different scanners.
 \\ \hline
 TUmor Proliferation Assessment Challenge 2016 (TUPAC16) - Mitosis \cite{124_veta2019cpath} & Prediction of a tumor proliferation score followed by mitotic counting & Type 1 & Three domains since the breast cancer cases were collected from three pathology labs \\
 \hline
 AIDPATH Kidney Database \cite{171_bueno2020cpath} & Detection and classificationof glomeruli & Type 1 & This dataset is composed of 5 different datasets from three different instituions.  \\
 \hline
 \multicolumn{4}{|c|}{\textbf{Classification}}\\
\hline
 Camelyon16 \cite{74_ehteshamibejnordi2017cpath} & Detection and classification of breast cancer metastases & Type 1 &  Two different domains since the whole slide images in the dataset were sourced from two pathology centres using two different scanners. \\
 \hline
Camelyon17 \cite{75_bandi2019cpath} & Detection and classification of breast cancer metastases & Type 1 & Five domains since the data was sourced from five different centres.  \\
\hline
PatchCamelyon benchmark \cite{76_veeling2018cpath} & Detection and classification of breast cancer metastases & Type 1 & Two domains since the data was sourced from two different centres. \\ 
\hline
Camelyon17-WILDS \cite{137_koh2021cpath} &  Detection and classification of breast cancer metastases & Type 1 & Five domains since the data was sourced from five different hospitals. \\
\hline
Lung and Colon Cancer Histopathological Image Dataset (LC25000) \cite{172_borkowski2019cpath} & Classification & Type 1 & Five domains with respect to cancer types and two domains with respect to organs. \\
\hline
Kather 19 \cite{173_kather2019cpath} & Colorectal tissue type classification & Type 1 & Three different domains with respect to centres.  \\
\hline
\multicolumn{4}{|c|}{\textbf{Segmentation}}\\
\hline
Multi-Organ Nucleus Segmentation Challenge (MoNuSeg) \cite{68_kumar2020cpath} & Nuclei instance segmentation & Type 1 & The dataset has 9 different domains with respect to organs and the training set has 18 different domains with respect to hospitals. \\
\hline
A Dataset for Nuclei Segmentation of Cryosectioned H\&E-stained Histological Images (CryoNuSeg) \cite{67_mahbod2021cpath} & Nuclei instance segmentation & Type 1, Type 3 & 10 domains (organs) with respect to domain shift type 1 and three domains with respect to domains shift type 3 as a consequence of three sets of manual mark-ups. \\
\hline
A Multi-Organ Nuclei Segmentation and Classification Challenge (MoNuSAC2020) \cite{73_verma2021cpath} & Nuclei instance segmentation and classification & Type 1, Type 2 & The dataset contains 37 domains with respect to hospitals, 71 domains with respect to patients and four domains with respect to organs.\\
\hline
The 2018 Data Science Bowl \cite{70_caicedo2019cpath} & Nucleus segmentation & Type 1, Type 4 & The dataset was sourced from 31 different imaing experiments representing 22 cell types and 5 groups of visually similar images across different modalities (brightfield vs. fluorescence).  \\
\hline
Crowdsource 2015 \cite{71_irshad2014cpath} & Nucleus detection and segmentation & Type 1, Type 3 & Six domains with respect to domain shift type 3. \\
\hline
CPM-17 \cite{69_vu2019cpath} & Nuclei instance segmentation & Type 1 & Four domain with respect to tissue images of four types of cancers. \\
\hline
PanNuke: An Open Pan-Cancer Histology Dataset for Nuclei Instance Segmentation and Classification \cite{66_gamper2020cpath} & Nuclei instance segmentation and classification & Type 1, Type 2 & 19 domains with respect to domain shift type 1 due to the presence of 19 different tissue types in the dataset. \\
\hline
Lizard: A large-scale dataset for colonic nuclear instance segmentation and classification \cite{72_graham2021cpath} & Nuclei instance segmentation and classification & Type 1, Type 3 & Six domain with respect to domain shift type 1 as the dataset includes data from six different sources (datasets). \\
\hline
Digestive-System Pathological Detection and Segmentation Challenge (DigestPath) 2019 \cite{125_da2022cpath} & Signet ring cell detection and Colonoscopy tissue segmentation and classification & Type 1 & Four domains as the dataset was sourced from four medical institutions. \\
\hline
MetaHistoSeg: A Python Framework for Meta Learning in Histopathology Image Segmentation \cite{45_yuan2021cpath} & Image segmentation &  Type 1 & Five domains as the dataset includes data from five different sources (datasets).\\
\hline
\end{longtable}
\footnotesize{'Type 1: Covariate Shift', 'Type 2: Prior Shift', 'Type 3: Posterior Shift', and 'Type 4: Class-Conditional Shift'}
\end{center}
\twocolumn

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


